Quantum Ensemble for Classification

A powerful way to improve performance in machine learning is to construct an ensemble that combines the predictions of multiple models. Ensemble methods are often much more accurate and lower variance than the individual classifiers that make them up but have high requirements in terms of memory and computational time. In fact, a large number of alternative algorithms is usually adopted, each requiring to query all available data. We propose a new quantum algorithm that exploits quantum superposition, entanglement and interference to build an ensemble of classification models. Thanks to the generation of the several quantum trajectories in superposition, we obtain $B$ transformations of the quantum state which encodes the training set in only $log\left(B\right)$ operations. This implies exponential growth of the ensemble size while increasing linearly the depth of the correspondent circuit. Furthermore, when considering the overall cost of the algorithm, we show that the training of a single weak classifier impacts additively the overall time complexity rather than multiplicatively, as it usually happens in classical ensemble methods. We also present small-scale experiments on real-world datasets, defining a quantum version of the cosine classifier and using the IBM qiskit environment to show how the algorithms work.

==> Figures/Encoding.tex <==
\begin{figure}
    \begin{minipage}{0.45\textwidth}
    \begin{algorithm}[H]
         \textbf{Training phase}
         \begin{enumerate}
             \item Initialize the parameters
             \begin{itemize}
                 \item $E=\emptyset$ the ensemble
                 \item $T$, Number of classifiers to train
             \end{itemize}
             \item For $t=1, \dots , T$
             \begin{itemize}
                 \item Take a bootstrap sample $D_t$ from $D$
                 \item Build a classifier $C_t$ using $D_t$ as training set
             \item Add the classifier to the current ensemble, $E = E \cup C_t$
             \end{itemize}
            \item Return $E$ \\
        \end{enumerate}
        \textbf{Testing phase}
        \begin{enumerate}[resume]
            \item Run $C_1, \dots C_T$ on the input $\tilde{x}$
            \item The class with highest probability is chosen as label for $\tilde{x}$
        \end{enumerate}
        \caption{Classical algorithm for bagging }
    \end{algorithm}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\textwidth}
    \begin{algorithm}[H]
        \textbf{State Preparation}
        \begin{enumerate}
            \item Initialize the quantum states
            \begin{itemize}
                \item Encoding: $D, \tilde{x} \rightarrow \ket{\psi}, \ket{\tilde{x}}$ \;
                \item Prepare $\ket{\phi}$
                \item Prepare $q$ ancilla qubits in uniform superposition
            \end{itemize}
     \end{enumerate}
     \textbf{Training + Test}
     \begin{enumerate}[resume]
         \item For $i = 2, 4, \dots, d$
         \begin{itemize}
             \item $c-swap(ctrl = anc_{i/2}, \ket{\psi}, \ket{\phi})$
             \item Apply $U_{i-1}$ to $\ket{\psi}$ and $U_{i}$ to $\ket{\phi}$  
             \item $c-swap(ctrl = anc_{i/2}, \ket{\psi}, \ket{\phi})$  
         \end{itemize}
     \item Apply $C$ to $\ket{\psi}$
     \end{enumerate}
     \textbf{Read out}
         \begin{itemize}
             %\item Take a bootstrap sample $D_t$ from $D$
             \item Measure the register of $\ket{\psi}$ which encodes $\tilde{y}$
         \end{itemize}
     %\item Return $E$ \\
        \caption{Quantum algorithm for bagging }
    \end{algorithm}
    \end{minipage}
    \caption{%\textbf{Comparison between quantum and classical bagging ensemble algorithm.} 
    Classical algorithm for bagging ensemble (left) includes two distinct steps, training and test. Their time complexity increases linearly on $T$. The training of a weak classifier and the number $T$ affect the most the whole time complexity of the algorithm. Quantum algorithm (right) does not require multiple uses of unitary $C$ (weak classifier) and depends linearly on $q = log(T)$. Its complexity is sensitive to the unitaries $U_i$, which in turn depends on the type of encoding for $D$. The overall complexity has to take into account also the state preparation routine and a readout step.}
    \label{pseudo-code}
\end{figure}

==> benchmark dataset/Encoding.tex <==
\begin{figure}
    \begin{minipage}{0.45\textwidth}
    \begin{algorithm}[H]
         \textbf{Training phase}
         \begin{enumerate}
             \item Initialize the parameters
             \begin{itemize}
                 \item $E=\emptyset$ the ensemble
                 \item $T$, Number of classifiers to train
             \end{itemize}
             \item For $t=1, \dots , T$
             \begin{itemize}
                 \item Take a bootstrap sample $D_t$ from $D$
                 \item Build a classifier $C_t$ using $D_t$ as training set
             \item Add the classifier to the current ensemble, $E = E \cup C_t$
             \end{itemize}
            \item Return $E$ \\
        \end{enumerate}
        \textbf{Testing phase}
        \begin{enumerate}[resume]
            \item Run $C_1, \dots C_T$ on the input $\tilde{x}$
            \item The class with highest probability is chosen as label for $\tilde{x}$
        \end{enumerate}
        \caption{Classical algorithm for bagging }
    \end{algorithm}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\textwidth}
    \begin{algorithm}[H]
        \textbf{State Preparation}
        \begin{enumerate}
            \item Initialize the quantum states
            \begin{itemize}
                \item Encoding: $D, \tilde{x} \rightarrow \ket{\psi}, \ket{\tilde{x}}$ \;
                \item Prepare $\ket{\phi}$
                \item Prepare $q$ ancilla qubits in uniform superposition
            \end{itemize}
     \end{enumerate}
     \textbf{Training + Test}
     \begin{enumerate}[resume]
         \item For $i = 2, 4, \dots, d$
         \begin{itemize}
             \item $c-swap(ctrl = anc_{i/2}, \ket{\psi}, \ket{\phi})$
             \item Apply $U_{i-1}$ to $\ket{\psi}$ and $U_{i}$ to $\ket{\phi}$  
             \item $c-swap(ctrl = anc_{i/2}, \ket{\psi}, \ket{\phi})$  
         \end{itemize}
     \item Apply $C$ to $\ket{\psi}$
     \end{enumerate}
     \textbf{Read out}
         \begin{itemize}
             %\item Take a bootstrap sample $D_t$ from $D$
             \item Measure the register of $\ket{\psi}$ which encodes $\tilde{y}$
         \end{itemize}
     %\item Return $E$ \\
        \caption{Quantum algorithm for bagging }
    \end{algorithm}
    \end{minipage}
    \caption{%\textbf{Comparison between quantum and classical bagging ensemble algorithm.} 
    Classical algorithm for bagging ensemble (left) includes two distinct steps, training and test. Their time complexity increases linearly on $T$. The training of a weak classifier and the number $T$ affect the most the whole time complexity of the algorithm. Quantum algorithm (right) does not require multiple uses of unitary $C$ (weak classifier) and depends linearly on $q = log(T)$. Its complexity is sensitive to the unitaries $U_i$, which in turn depends on the type of encoding for $D$. The overall complexity has to take into account also the state preparation routine and a readout step.}
    \label{pseudo-code}
\end{figure}

==> benchmark dataset/circuit_ensemble.tex <==
\Qcircuit @C=.8em @R=.8em {
& & \hspace{2.8em}  & &  \hspace{4.3em} \ket{\Phi_{0}} &  &&& \hspace{-3.2em} \ket{\Phi_{1}} & &&& \hspace{-2em} \ket{\Phi_{2}} & &&& \hspace{-10em} \ket{\Phi_{d-1}} & & \hspace{-1em} \ket{\Phi_{d}} \\
\lstick{1} 
 &&& \lstick{\ket{0}}  & \multigate{3}{W} 
\ar@{--}[]+<2.em,.5em>;[d]+<2.em,-7.5em> 
& \qw & \qw   & \qw 
\ar@{--}[]+<1.8em,.5em>;[d]+<1.8em,-7.5em> 
& \qw & \qw & \qw 
\ar@{--}[]+<2.em,.5em>;[d]+<2.em,-7.5em>  
& \qw & \qw  
\ar@{--}[]+<2.em,.5em>;[d]+<2.em,-7.5em>   
& \qw & \qw  & \ctrl{4}& \gate{X}& \ctrl{4} 
\ar@{--}[]+<2.em,.5em>;[d]+<2.em,-7.5em>   
& \qw &&  
\\
 &&& \lstick{\dots} & \ghost{W} & \qw & \qw & \qw & \qw & \qw & \qw & \qw  & \qw & \qw  & \qw & \qw & \qw & \qw & \qw  \\
\lstick{d-1}  &&& \lstick{\ket{0}} & \ghost{W} & \qw & \qw & \qw & \ctrl{2}   & \gate{X}  & \ctrl{2} & \qw  & \qw & \qw & \qw & \qw & \qw & \qw & \qw \\
\lstick{d}  &&& \lstick{\ket{0}}  & \ghost{W} & \ctrl{1} & \gate{X} & \ctrl{1} & \qw & \qw & \qw & \qw  & \cdots && \qw & \qw & \qw & \qw  & \qw \hspace{6.5em} \ket{\Phi_{f}} \\
\lstick{data}  &&& \lstick{\ket{0}}    & \gate{S_{(x,y)}} & \gate{U_{(1,1)})} & \qw & \gate{U_{(1,2)}}& \gate{U_{(2,1)}}& \qw & \gate{U_{(2,2)}}& \qw  & \cdots && \qw & \gate{U_{(d,1)}}& \qw & \gate{U_{(d,2)}} & \qw & \multigate{2}{F} \ar@{--}[]+<1.6em,1em>;[d]+<1.6em,-3em>  
 \\
& & & & & & & & & & & & & & & \lstick{test} &  \lstick{\ket{0}} & \multigate{1}{S_{(x^{(\text{test})},0)}} & \qw & \ghost{F} & \qw &\meter\\
& & & & & & & & & & & & & & & &  \lstick{\ket{0}} & \ghost{S_{(x^{(\text{test})},0)}} & \qw & \ghost{F}
}


